Higher-Order Analysis of Three-Dimensional Anisotropy in Imbalanced Alfv\'enic Turbulence

We analyze in-situ observations of imbalanced solar wind turbulence to evaluate MHD turbulence models grounded in "Critical Balance" (CB) and "Scale-Dependent Dynamic Alignment" (SDDA). At energy injection scales, both outgoing and ingoing modes exhibit a weak cascade; a simultaneous tightening of SDDA is noted. Outgoing modes persist in a weak cascade across the inertial range, while ingoing modes shift to a strong cascade at $\lambda \approx 3 \times 10^{4} d_i$, with associated spectral scalings deviating from expected behavior due to "anomalous coherence" effects. The inertial range comprises two distinct sub-inertial segments. Beyond $\lambda \gtrsim 100 d_i$, eddies adopt a field-aligned tube topology, with SDDA signatures mainly evident in high amplitude fluctuations. The scaling exponents $\zeta_{n}$ of the $n$-th order conditional structure functions, orthogonal to both the local mean field and fluctuation direction, align with the analytical models of Chandran et al. 2015 and Mallet et al. 2017, indicating "multifractal" statistics and strong intermittency; however, scaling in parallel and displacement components is more concave than predicted, possibly influenced by expansion effects. Below $\lambda \approx 100 d_i$, eddies become increasingly anisotropic, evolving into thin current sheet-like structures. Concurrently, $\zeta_{n}$ scales linearly with order, marking a shift towards "monofractal" statistics. At $\lambda \approx 8 d_i$, the increase in aspect ratio halts, and the eddies become quasi-isotropic. This change may signal tearing instability, leading to reconnection, or result from energy redirection into the ion-cyclotron wave spectrum, aligning with the "helicity barrier". Our analysis utilizes 5-point structure functions, proving more effective than the traditional 2-point method in capturing steep scaling behaviors at smaller scales.

==> notes.tex <==
Conversely, in homogeneous simulations of \cite{2023_Chen_compres}, the balanced runs exhibited better alignment with the scaling predictions of \citetalias{chandran_intermittency_2015} and \citetalias{Mallet_2017}, consistent with prior numerical studies of balanced RMHD turbulence \citep{chandran_intermittency_2015, 2016_mallet}.


The lower panels of the figure display the absolute values of the local scaling index, calculated over the interval ($\ell/\sqrt{w}, ~ \ell\sqrt{w}$) with $w=3$. For ease of comparison, reference lines corresponding to scaling indices $\gamma$ = 0, 1/3, 2/3, and 1 are included. Furthermore,

The lower panels illustrate the absolute value of the local scaling index corresponding to the color-matched curves in the upper panels, alongside reference lines at $\gamma = ~0, ~1/3, ~2/3, ~1$.

 predicts a alignment in  Els\"asser fluctuations, which emerges from strongly imbalanced collisions of counter-propagating wavepackets. Therefore, despite certain limitations, the model inherently incorporates the concept of local imbalance. This is due to the dynamical alignment in polarizations that arises from these highly imbalanced collisions of counterpropagating wavepackets.

To estimate the Els\"asser variables, we interpolate the magnetic field data to align with the temporal resolution of the ion moment data and use a 30-second moving average for the proton density, $n_p$.


Note,  that when utilizing two-point structure functions-- as opposed to the five-point structure functions shown here-- the scaling exponents obtained for the parallel component of the magentic field are in agreement with those reported in  \citep{Wu2022OnTS}







Therefore, selecting extended homogeneous intervals for analysis is imperative to extract meaningful results and accurately represent the inherent variability in solar wind turbulence.

who further emphasized that CB, often perceived as a core framework in incompressible MHD, is in fact a model that emerges from a succession of approximations and physical arguments. They 





 As it is well known, SFs obey power-laws with respect to the different scales, as $SF_{i}^{n}(\ell)\propto\ell^{\zeta(n)}$. These scaling exponents are in general a function of the moment order n. The scaling exponents provide the opportunity to test the different turbulence and intermittency models. For instance, the K41 and IK paradigms predict constant scalings:
\begin{equation}
    \zeta^{K41}(n)=\frac{n}{3}\quad \& \quad \zeta^{IK}(n)=\frac{n}{4}
    \label{eq:3}
\end{equation}
indicative of self-similar (not intermittent) behaviour. Since results both from RMHD simulations and solar wind observations showed the presence of intermittency in the inertial range of turbulence, both these models where refined to include multi-fractallity, by Horbury \& Balogh (1997) and Politano \& Pouquet (1995) respectively.



It’s important to note that the estimates of $\tau_{nl}$ in \cite{Chhiber_2020_timescales} are based on a global magnetic field measurement approach, contrasting with the locally defined field method used in \cite{2015Mallet}



To investigate the 3D anisotropic nature of the magnetic field in the inner heliosphere, we calculate the five-point structure functions of the magnetic field fluctuations \citep{cho} in each spatial dimension. Specifically, the five-point SFs of order-n, at scale $\boldsymbol{\ell}$ are  defined as:
\begin{equation}
\begin{split}
      SF_{i}^{n}(\boldsymbol{\ell})=&\langle |[\delta \boldsymbol{B_{i}}(\boldsymbol{r}-2\boldsymbol{\ell})-4\delta \boldsymbol{B_{i}}(\boldsymbol{r}-\boldsymbol{\ell})+6\delta \boldsymbol{B_{i}}(\boldsymbol{r})\\&-4\delta \boldsymbol{B_{i}}(\boldsymbol{r}+\boldsymbol{\ell})+\delta \boldsymbol{B_{i}}(\boldsymbol{r}+2\boldsymbol{\ell})]/\sqrt{35}|^n\rangle_{r}
      \label{eq:2}
\end{split}      
\end{equation}
where $\boldsymbol{i}=\boldsymbol{l_{\parallel}}, \boldsymbol{l_{\perp}}, \boldsymbol{L_{\perp}}$ and $\langle...\rangle_{r}$ denotes a spatial ensemble average (associated with the interval duration).  is a more detailed and sensitive estimation of the information contained in the structure functions and their scaling -besides, the applicability of this method to kinetic scales will be questioned in this study.











% It is important to note that both \citetalias{chandran_intermittency_2015} and \citetalias{Mallet_2017}, along with \citetalias{goldreich_toward_1995} and \citetalias{boldyrev_2006}, theories assume a balance between the energies of the two Els\"asser fields ($\delta\boldsymbol{z}^{+} \sim \delta\boldsymbol{z}^{-}$), implying negligible cross helicity.


% In order to preform the analysis presented in this letter reliably, we firstly divided our dataset into 3h-long intervals. We, then, went one to estimate the five-point SFs and the resulting scaling exponents in the inertial range. In an attempt to increase the sensitivity of the SF scaling calculation at the kinetic scales, the Continuous Wavelet Transform (CWT) approach was applied. Having obtained these results, we evaluated the empirical PDFs and found for the first time the most appropriate fit amongst the 89 most known distributions in Mathematics, in all turbulent scales. Using the integral (\ref{eq:5}) we appraisaled the SFs and compared with our previous results. This analysis was attained for all three spatial dimensions. In each case we distinguished the fast and slow streams of the wind, with the threshold of $400 \, km/sec$.

% In the first step, we used equation (\ref{eq:2}) to determine the five-point SFs for the three anisotropic dimensions of the high-resolution dataset, from PSP's 1st encounter (hereafter E1). The graphs presented are based on $80$ estimated points (trough (\ref{eq:2})), on a range from the kinetic scales all the way to the energy injection scales. The angle thresholds for each dimension, are also presented in the figures. It is clear from Figure \ref{}, that until $\ell[d_i]\propto10^{-4}$ the condition $SF^2_{l_{\perp}}>SF^2_{l_{\perp}}>SF^2_{l_{\parallel}}$ is satisfied, which was previously demonstrated only for the kinetic scales of turbulence in the inner heliosphere (Zhang et al. \ref{}). Our results indicate the extended presence of 3D anisotropy in the inertial range and also the well-known fact that the perpendicular fluctuations determine the behavior of the energy cascade towards smaller scales\footnote{This can also be identified from the empirical SFs shown later, where the values of the SFs belonging in the perpendicular plane are greater in each scale.}. Moreover, paradoxically for a good part of the inertial range, the perpendicular scales exhibit similar behavior and someone could argue 2D anisotropy in the inertial and dissipation range (???).  At even greater scales, it is evident that the three curves of the structure functions tend to align, because of the fact that the anisotropy has not been developed yet. We then went on to plot the first $8$ moment orders of the magnetic field increments, and apply the appropriate power law fits to extract the various scalings -shown in Figure \ref{}. As expected, the resolution of orders higher than $4$ is diminished, making them unreliable (the tails of the distributions do not drop to zero fast enough, i.e. Palacios et al. \ref{}). This is also reflected at kinetic scales (specifically beyond $10^0\,d_i$), where the five-point SF method is perhaps untrustworthy considering the spacecraft reaction wheels noise (Duan et al. \ref{}).  Besides, the scaling exponents are much alike the predictions of CH15 (within the approximated error), especially in the perpendicular plane (??). This is indicative of the validity of this model, even in situations of imbalanced turbulence -as in very close to the Sun. In all cases, the deviation from self-similarity is clear, as the cascade is multifractal. 

% Following the same procedure, the calculation of the five-point SFs for the mixed dataset (containing highly alfvenic $0.75<\sigma_c<1$ slow wind data from the first $13$ perihelions of PSP, with heliocentric distances $34R_o<R<63R_o$) resulted in the structure functions shown in Figure \ref{}. The quality assets of the high order SFs are similar to the E1 case, whilst the disturbances -for instance in $\bf{\ell}$- could very well be ascribed to the more strict data demands\footnote{We attempted to find as long slow wind intervals as possible, being highly Alfv{\'e}nic.}. These additional constraints provide extra limitations to the dataset, ensuring though that we are studying a specific type of wind. The scalings are following once again the CH15 paradigm. For the parallel direction, the deviation arises from the fact that the higher order structure functions do not saturate, making it extremely difficult to find an appropriate linear fit over the same range of scales as in lower SFs.


\subsection{Scale-Dependent Kurtosis}\label{subsec:SDK}

Another good way to examine the intermittent behaviour of a timeseries is through the so called Scale-Dependent Kurtosis (hereafter SDK), which is a normalised fourth-order moment and can be defined as:
\begin{equation}\label{eq:20}
    \kappa(\ell)=\frac{SF^4_i(\ell)}{[SF^2_i(\ell)]^2}.
\end{equation}
This can be thought as a measure of intermittency, since self-similarity is depicted on a constant value of the SDK -irrespective of scale (i.e. the probability distributions of the fluctuations collapse to a unique PDF, after different rescalings). A multifractal cascade, on the other hand, is represented by a progressively increasing SDK towards smaller scales.
As it is well known, a Gaussian distribution is characterised by a constant value $\kappa(\ell)=3$. An oscillation around a certain value is in general indicative of a monofractal behaviour, in this case Super-Gaussian. Moreover, multi-fractal cascades arise from the fact that the distributions of the fluctuations at smaller scales exhibit progressively fatter tails (\ref{} Frisch 1995). 



Having explained the necessity of the 5-point structure functions, we move on to discuss the behaviour of SDK$_{5}$. It is apparent, first of all, that one cannot define with clarity one inertial range. Both regions $R_1$ and $R_2$ satisfy a scaling, and it is quite plausible to argue that even the intermediate region follows a (different) scaling. Hence, we observe multiple sub-inertial ranges and this could be assigned to the fact that near the Sun the turbulent regime is not yet fully developed. 





  

While 



\footnote{In contrast, the solar wind shows an inertial scaling shift from $a_{\perp} = -3/2$ at $|\sigma_c| \rightarrow 0$ to $a_{\perp} = -5/3$ at $|\sigma_c| \rightarrow 1$ \citep{Podesta_2010, Chen_2013, sioulas_turb_22_no1}. Unlike numerical experiments, which are largely incompressible, solar wind compressibility closely correlates with imbalance. This suggests that compressibility, rather than imbalance, might dictate the inertial range scaling \citep{Wang_2023, 2023_Dunn}.}

 A common limitation of MHD simulations is their low resolution, which aligns their scaling exponents predominantly with the $R_2$ scale range.




\subsection{Limitations }\label{subsec:limitations}



\par At this point, it is imperative to acknowledge certain limitations associated with the analysis presented in this work.

\par First and foremost, as stressed in several points 



Second-order, 5-pt structure functions ($SF_{5}^{2}$) for parallel, perpendicular, and displacement components were computed according to Equations \ref{eq:20} - \ref{eq:22}. Following the approach of \citet{Chen_2012ApJ}, each interval's $SF_{5}^{2}$ was normalized by $\langle |\boldsymbol{B}|^{2} \rangle$. The dataset's average, $\tilde{SF}_{5}^{2}$, was computed utilizing 120 linearly spaced bins in logarithmic space, with the weighting for each bin corresponding to the number of increments at that scale within the respective interval.






\par Figure \ref{fig:1} presents the findings of the analysis. In the top panels (a), (c), and (e), $\tilde{SF}_{5}^{2}$ for the parallel, perpendicular, and displacement components are plotted against scales in ion inertial length units ($d_i$). To facilitate comparison, each panel includes reference power-law lines for $\beta = 1/2, 2/3, 1$, corresponding to spectral indices $\alpha_{B} = -1-\beta$ \citep{monin_statistical_1987}.

However, further work is needed on several fronts. Firstly, a more detailed analysis is required, which involves estimating 3D anisotropic structure functions while taking into account the angle between $\delta v_{sc}$ and $\boldsymbol{B}_{0}$. Such an analysis will enable us to consider the effects of the sampling direction on anisotropic statistics. Secondly, EBM numerical simulations analyzing 3D anisotropy, and higher-order statistics should incorporate factors such as imbalance, more comprehensively. This would involve conducting a larger number of simulation runs, particularly those under realistic Parker Spiral conditions. These comprehensive simulations are essential for deepening our understanding of these complex systems and confirming the applicability of existing theoretical models.




Given that high-quality, high-resolution data are only available for highly Alfv\'enic imbalanced turbulence during E1 of PSP, it is crucial to consider the potential impact of balanced intervals on our results.


The near-Sun solar wind environment is characterized by the ubiquitous presence of Switchbacks, a subset of largely Alfv\'enic fluctuations whose amplitude is sufficiently large to cause the magnetic field to kink backwards on itself \citep{Matteini_2014}. This kinking results in a local field polarity reversal and a corresponding radial velocity jet  \citep{2018_horbury_switchbacks, bale_highly_2019,dudok_de_wit_switchbacks_2020, martinovic_multiscale_2021, 2021_larosa,Tenerani_2021,Shi_2022_patches}. Such sudden revearsals could result in large uncertainties in the direction analysis




In light of the five caveats discussed above, it becomes clear that further detailed analysis of this problem is necessary. Nevertheless, our method has, for the first time, 




 Given the potential quality issues with velocity data necessary for estimating Els\"asser variables, we proceed with caution, mindful that such issues could introduce further uncertainties to our analysis.



 However, the accuracy of these $R_1$ results is debatable. Small errors in velocity measurements, which are accentuated at smaller scales, can lead to significant uncertainties in the calculated alignment angles, as highlighted by \citep{Podesta_2010}


When employing the same methodology, corroborates this result, with $\chi_{\lambda} \sim 1$, as illustrated by the gray line in Figure \ref{fig:5}c. However, when applying the definition that incorporates alignment, we observe that $\chi_{\xi} \geq 1$ for $\lambda \geq 100 d_i$, but the non-linearity parameter drops below unity, $\chi_{\xi} < 1$, in $R_1$.


 Initially, in line with the methodology of \citep{chen_2016}, we 
\par 





 \par The data suggest that while turbulence is strong at large scales, it weakens gradually, with the nonlinearity parameter $\chi$ dropping below 1 at $\lambda \approx 100 d_i$. This threshold marks the beginning of the sub-inertial range, $R_1$.

The scale-dependent behavior of $\chi^{\pm}$ is contingent upon the definition considered, i.e., either $\chi^{\pm}_{\lambda}$ or $\chi^{\pm}_{\xi}$.
